A Hybrid Approach to Query Answering under Expressive Datalog+/-

Datalog+/- is a family of ontology languages that combine good computational properties with high expressive power. Datalog+/- languages are provably able to capture the most relevant Semantic Web languages. In this paper we consider the class of weakly-sticky (WS) Datalog+/- programs, which allow for certain useful forms of joins in rule bodies as well as extending the well-known class of weakly-acyclic TGDs. So far, only non-deterministic algorithms were known for answering queries on WS Datalog+/- programs. We present novel deterministic query answering algorithms under WS Datalog+/-. In particular, we propose: (1) a bottom-up grounding algorithm based on a query-driven chase, and (2) a hybrid approach based on transforming a WS program into a so-called sticky one, for which query rewriting techniques are known. We discuss how our algorithms can be optimized and effectively applied for query answering in real-world scenarios.

==> macros.tex <==
\newcommand{\keywords}[1]{\par\addvspace\baselineskip
\noindent\keywordname\enspace\ignorespaces#1}

\newcounter{rownum}
\newcommand{\mc}[1]{\mathcal{ #1}}
\newcommand{\nit}[1]{{\it #1}}
\newcommand{\boxtheorem}{\hfill $\Box$\vspace*{0.2cm}}
\newcommand{\ignore}[1]{}
\newcommand{\defproof}[2]{{\noindent\bf Proof of #1:\
}#2 \boxtheorem\\ \vspace{2mm}}
\newenvironment{lemmaA}%
{\vskip \abovedisplayskip \refstepcounter{lemmaA-counter}%
\noindent {\bf Lemma A.\arabic{lemmaA-counter}.}}%

\newcounter{lemmaA-counter}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\comlb}[1]{{\vspace{2mm}\noindent \bf \red{COMM(LEO):}}~ #1 \hfill {\bf
    END.}\\}
\newcommand{\commos}[1]{{\vspace{2mm}\noindent \bf \blue{COMM(MOSTAFA):}}~ #1 \hfill {\bf
    END.}\\}


\newcommand{\datalogpm}{Datalog$^\pm$}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

